Clustering in Block Markov Chains

This paper considers cluster detection in Block Markov Chains (BMCs). These Markov chains are characterized by a block structure in their transition matrix. More precisely, the $n$ possible states are divided into a finite number of $K$ groups or clusters, such that states in the same cluster exhibit the same transition rates to other states. One observes a trajectory of the Markov chain, and the objective is to recover, from this observation only, the (initially unknown) clusters. In this paper we devise a clustering procedure that accurately, efficiently, and provably detects the clusters. We first derive a fundamental information-theoretical lower bound on the detection error rate satisfied under any clustering algorithm. This bound identifies the parameters of the BMC, and trajectory lengths, for which it is possible to accurately detect the clusters. We next develop two clustering algorithms that can together accurately recover the cluster structure from the shortest possible trajectories, whenever the parameters allow detection. These algorithms thus reach the fundamental detectability limit, and are optimal in that sense.

==> Chapter__Concentration_of_spectral_norm.tex <==
\chapter{Concentration of the spectral norm of the noise matrix}
\label{sec:Open_problem}

Recall that the Spectral Clustering Algorithm and Cluster Improvement Algorithm rely on calculating the matrices $\hat{N} \in \naturalNumbersZero^{n \times n}$ and $\hat{P} \in \DDelta^{(n-1) \times n}$ element-wise as
\begin{equation}
\hat{N}_{x,y}
= \sum_{t=0}^{T-1} \indicator{ X_t = x, X_{t+1} = y },
%\quad
%\textrm{and}
%\quad
\,
\hat{P}_{x,y}
= \frac{ \sum_{t=0}^{T-1} \indicator{ X_t = x, X_{t+1} = y } }{ \sum_{t=0}^{T-1} \indicator{ X_t = x } }
%\quad
%\textrm{for}
%\quad
\, \forall_{x,y} \in \mathcal{V}. 
\nonumber
\end{equation} 
In the convergence proofs of the algorithms, we encountered the spectral norms of the noise matrices $\hat{N} - N$ and $\hat{P} - P$. Specifically, we require that $\pnorm{ \hat{N} - N }{}$ is atleast $\smallOP{T/n}$ and $\pnorm{ \hat{P} - P }{}$ atleast $\smallOP{1}$. The primary difficulty in proving these statements though is that $\hat{N}$ constitutes a random matrix with stochastic \emph{dependent} entries. While concentration of the eigenvalues of a random matrix has been actively investigated when the entries are independent or satisfy a weak condition of dependence \cite{wigner_distribution_1958,tao_topics_2012,tropp_introduction_2015,hochstattler_semicircle_2016,kirsch_sixty_2016,kirsch_semicircle_2017}, or when the transition matrix of the Markov chain itself is random \cite{bordenave_spectrum_2010,bordenave_spectrum_2011}, we were unable to find work relating to the case when the entries are dictated by a Markov chain with a fixed transition matrix with a block structure. 

We therefore examined proof strategies to obtain bounds on the concentration of $\pnorm{ \hat{N} - N }{}$ and $\pnorm{ \hat{P} - P }{}$, each with varying degrees of success. These included an attempt to reduce the problem to a case of independent entries \cite{coja-oghlan_graph_2010}, applying an epsilon-net argument \cite{tao_topics_2012}, Wigner's trace method \cite{wigner_distribution_1958,vu_spectral_2005}, Stein's method for concentration inequalities \cite{chatterjee_steins_2007}, generalized Hoeffding inequalities for Markov chains \cite{glynn_hoeffding_2002,boucher_hoeffding_2009,chung_chernoff_2012}, matrix perturbation techniques \cite{bauer_norms_1960,chu_generalization_1986,haviv_taylor_1992,meyer_sensitivity_1994}, and a method of exchangeable pairs \cite{mackey_matrix_2014}. We give this (nonexhaustive) list of approaches to facilitate future research, because while we have so far been unable to prove the following conjecture, we believe it holds and warrants further investigation. 

\begin{conjecture}
\label{conjecture:Concentration_of_Nhat_to_N}
If the Markov chain $\process{X_t}{t \geq 0}$ is a \gls{BMC} and $T = \omega(n)$, then there exist functions $f(n,T) = \smallO{T/n}$ and $g(n,T) = \smallO{1}$ such that $\pnorm{ \hat{N} - N }{} = \bigOP{ f(n,T) }$ and $\pnorm{ \hat{P} - P }{} = \bigOP{ g(n,T) }$, respectively.
\end{conjecture}

We verified numerically that the above conjecture holds. In Figure \ref{fig:Asymptotic_behavior_of_spectral_norm_Nhat_minus_N}, we plot  $\pnorm{ \hat{N} - N }{}$ as a function of the number $n$ of states. The results reported there suggest that the conjecture holds for $f(n,T) \approx \sqrt{T/n}$.  
\begin{figure}[!hbtp]
\centering
\begin{subfigure}[t]{0.3\textwidth}
\centering
\begin{tikzpicture}[scale=0.475]
\begin{axis}[
	xmin = 50, xmax = 550,
	xtick = {100,200,300,400,500},
	ymin = 0, ymax = 75,
	ytick = {0,25,50,75},
	xlabel=$n$, ylabel={$\pnorm{ \hat{N} - N }{}$},
	anchor = origin
]

\addplot[mark=x,only marks,error bars/.cd, y dir=both, y explicit] plot coordinates {
	(100.,15.4315) += (100.,1.49844) -= (100.,1.49844)
	(110.,16.3849) += (110.,1.41984) -= (110.,1.41984)
	(120.,15.8832) += (120.,1.21284) -= (120.,1.21284)
	(130.,16.572) += (130.,0.947396) -= (130.,0.947396)
	(140.,17.0106) += (140.,1.04959) -= (140.,1.04959)
	(150.,16.982) += (150.,0.893277) -= (150.,0.893277)
	(160.,18.5368) += (160.,1.36868) -= (160.,1.36868)
	(170.,17.9443) += (170.,0.917998) -= (170.,0.917998)
	(180.,19.0965) += (180.,1.40359) -= (180.,1.40359)
	(190.,17.9435) += (190.,0.681452) -= (190.,0.681452)
	(200.,18.3453) += (200.,0.843741) -= (200.,0.843741)
	(210.,18.4662) += (210.,0.822152) -= (210.,0.822152)
	(220.,19.1497) += (220.,1.24501) -= (220.,1.24501)
	(230.,18.7638) += (230.,0.822557) -= (230.,0.822557)
	(240.,19.1394) += (240.,0.615285) -= (240.,0.615285)
	(250.,20.3555) += (250.,1.08903) -= (250.,1.08903)
	(260.,19.3521) += (260.,0.671457) -= (260.,0.671457)
	(270.,20.3161) += (270.,1.23526) -= (270.,1.23526)
	(280.,19.4939) += (280.,0.734102) -= (280.,0.734102)
	(290.,20.2258) += (290.,1.03484) -= (290.,1.03484)
	(300.,20.1788) += (300.,0.840964) -= (300.,0.840964)
	(310.,20.9089) += (310.,0.932142) -= (310.,0.932142)
	(320.,20.2316) += (320.,0.955103) -= (320.,0.955103)
	(330.,20.7617) += (330.,0.742022) -= (330.,0.742022)
	(340.,21.2145) += (340.,0.77354) -= (340.,0.77354)
	(350.,20.2486) += (350.,0.843586) -= (350.,0.843586)
	(360.,21.3489) += (360.,0.928621) -= (360.,0.928621)
	(370.,21.2754) += (370.,1.16943) -= (370.,1.16943)
	(380.,20.8849) += (380.,0.867949) -= (380.,0.867949)
	(390.,21.3546) += (390.,1.10446) -= (390.,1.10446)
	(400.,21.639) += (400.,0.762752) -= (400.,0.762752)
	(410.,21.8068) += (410.,0.728122) -= (410.,0.728122)
	(420.,21.8224) += (420.,0.970879) -= (420.,0.970879)
	(430.,22.7728) += (430.,1.22447) -= (430.,1.22447)
	(440.,22.7045) += (440.,0.928033) -= (440.,0.928033)
	(450.,22.2249) += (450.,0.807621) -= (450.,0.807621)
	(460.,21.6465) += (460.,0.791279) -= (460.,0.791279)
	(470.,22.6298) += (470.,0.741794) -= (470.,0.741794)
	(480.,22.5865) += (480.,0.766488) -= (480.,0.766488)
	(490.,21.9972) += (490.,0.685546) -= (490.,0.685546)
	(500.,22.9296) += (500.,0.691819) -= (500.,0.691819)
} node [above=45, anchor=east] {Case $T = n (\ln{n})^{3/2}$ \quad};
\addplot[domain=100:500]{-12.6562+8.95248*sqrt(ln(x)^1.5)} node [below=60, anchor=east] {};% {Fit $-13+9\sqrt{ ( \ln{n} )^{3/2} }$};


\addplot[mark=x,only marks,error bars/.cd, y dir=both, y explicit] plot coordinates {
	(100.,30.6307) += (100.,1.91138) -= (100.,1.91138)
	(110.,34.1932) += (110.,2.81114) -= (110.,2.81114)
	(120.,34.512) += (120.,2.40415) -= (120.,2.40415)
	(130.,35.9862) += (130.,3.33096) -= (130.,3.33096)
	(140.,39.7799) += (140.,4.07264) -= (140.,4.07264)
	(150.,37.3359) += (150.,3.17701) -= (150.,3.17701)
	(160.,41.5088) += (160.,2.98241) -= (160.,2.98241)
	(170.,39.5388) += (170.,2.85831) -= (170.,2.85831)
	(180.,37.6244) += (180.,2.38669) -= (180.,2.38669)
	(190.,39.4319) += (190.,1.94155) -= (190.,1.94155)
	(200.,38.9327) += (200.,1.28428) -= (200.,1.28428)
	(210.,42.0987) += (210.,2.8327) -= (210.,2.8327)
	(220.,40.5954) += (220.,1.61212) -= (220.,1.61212)
	(230.,41.8787) += (230.,2.12044) -= (230.,2.12044)
	(240.,42.331) += (240.,2.80018) -= (240.,2.80018)
	(250.,46.161) += (250.,3.04052) -= (250.,3.04052)
	(260.,45.1146) += (260.,2.46119) -= (260.,2.46119)
	(270.,45.3518) += (270.,2.10076) -= (270.,2.10076)
	(280.,45.7441) += (280.,2.34707) -= (280.,2.34707)
	(290.,47.3855) += (290.,2.28878) -= (290.,2.28878)
	(300.,47.0722) += (300.,1.69757) -= (300.,1.69757)
	(310.,45.1731) += (310.,0.913772) -= (310.,0.913772)
	(320.,47.3447) += (320.,1.53119) -= (320.,1.53119)
	(330.,47.9021) += (330.,1.93297) -= (330.,1.93297)
	(340.,49.133) += (340.,1.87986) -= (340.,1.87986)
	(350.,49.6063) += (350.,1.73457) -= (350.,1.73457)
	(360.,49.8737) += (360.,2.32802) -= (360.,2.32802)
	(370.,49.1985) += (370.,1.86958) -= (370.,1.86958)
	(380.,50.6349) += (380.,1.71719) -= (380.,1.71719)
	(390.,51.4565) += (390.,2.22502) -= (390.,2.22502)
	(400.,51.2219) += (400.,2.27438) -= (400.,2.27438)
	(410.,51.7979) += (410.,2.03744) -= (410.,2.03744)
	(420.,51.9531) += (420.,2.35978) -= (420.,2.35978)
	(430.,52.2133) += (430.,2.02262) -= (430.,2.02262)
	(440.,53.5652) += (440.,2.33912) -= (440.,2.33912)
	(450.,54.5599) += (450.,2.3776) -= (450.,2.3776)
	(460.,51.6383) += (460.,1.72589) -= (460.,1.72589)
	(470.,53.7351) += (470.,1.80685) -= (470.,1.80685)
	(480.,53.9907) += (480.,2.21706) -= (480.,2.21706)
	(490.,54.4568) += (490.,2.17541) -= (490.,2.17541)
	(500.,55.3777) += (500.,2.04061) -= (500.,2.04061)
} node [above=45, anchor=east] {Case $T = n (\ln{n})^{2}$ \quad};
\addplot[domain=100:500]{-33.0135+14.0454*sqrt(ln(x)^2)} node [below=90, anchor=east] {};% {Fit $-33+14\sqrt{ ( \ln{n} )^2 }$};
\end{axis}
\end{tikzpicture}
\end{subfigure}
~
\begin{subfigure}[t]{0.3\textwidth}
\centering
\begin{tikzpicture}[scale=0.475]
\begin{axis}[
	xmin = 50, xmax = 550,
	xtick = {100,200,300,400,500},
	ymin = 0, ymax = 750,
	ytick = {0,250,500,750},
	xlabel=$n$,% ylabel={$\pnorm{ \hat{N} - N }{}$},
	anchor = origin,
	label style={font=\Large},
	tick label style={font=\Large}	
]

\addplot[mark=x,only marks,error bars/.cd, y dir=both, y explicit] plot coordinates {
	(100.,149.144) += (100.,15.6162) -= (100.,15.6162)
	(110.,155.662) += (110.,10.4643) -= (110.,10.4643)
	(120.,178.164) += (120.,10.6258) -= (120.,10.6258)
	(130.,192.453) += (130.,16.5378) -= (130.,16.5378)
	(140.,202.218) += (140.,14.9712) -= (140.,14.9712)
	(150.,201.523) += (150.,13.3947) -= (150.,13.3947)
	(160.,225.157) += (160.,13.8526) -= (160.,13.8526)
	(170.,251.744) += (170.,14.6015) -= (170.,14.6015)
	(180.,251.499) += (180.,11.9138) -= (180.,11.9138)
	(190.,274.968) += (190.,13.371) -= (190.,13.371)
	(200.,297.273) += (200.,19.3186) -= (200.,19.3186)
	(210.,307.326) += (210.,16.1287) -= (210.,16.1287)
	(220.,317.037) += (220.,13.2915) -= (220.,13.2915)
	(230.,313.776) += (230.,10.4709) -= (230.,10.4709)
	(240.,346.047) += (240.,14.6914) -= (240.,14.6914)
	(250.,337.125) += (250.,14.1132) -= (250.,14.1132)
	(260.,355.773) += (260.,17.7606) -= (260.,17.7606)
	(270.,382.025) += (270.,23.7126) -= (270.,23.7126)
	(280.,391.376) += (280.,19.9914) -= (280.,19.9914)
	(290.,420.035) += (290.,17.3563) -= (290.,17.3563)
	(300.,426.953) += (300.,18.1754) -= (300.,18.1754)
	(310.,431.342) += (310.,17.1745) -= (310.,17.1745)
	(320.,473.402) += (320.,23.1998) -= (320.,23.1998)
	(330.,461.708) += (330.,20.4388) -= (330.,20.4388)
	(340.,475.89) += (340.,18.6793) -= (340.,18.6793)
	(350.,508.384) += (350.,24.0685) -= (350.,24.0685)
	(360.,494.781) += (360.,17.8275) -= (360.,17.8275)
	(370.,509.487) += (370.,19.9116) -= (370.,19.9116)
	(380.,518.127) += (380.,22.8355) -= (380.,22.8355)
	(390.,523.94) += (390.,17.3776) -= (390.,17.3776)
	(400.,571.738) += (400.,29.4008) -= (400.,29.4008)
	(410.,597.894) += (410.,29.2037) -= (410.,29.2037)
	(420.,592.338) += (420.,24.7825) -= (420.,24.7825)
	(430.,610.625) += (430.,27.5173) -= (430.,27.5173)
	(440.,605.314) += (440.,34.8579) -= (440.,34.8579)
	(450.,629.299) += (450.,30.0859) -= (450.,30.0859)
	(460.,650.861) += (460.,20.2152) -= (460.,20.2152)
	(470.,640.684) += (470.,22.561) -= (470.,22.561)
	(480.,679.057) += (480.,29.7178) -= (480.,29.7178)
	(490.,690.217) += (490.,20.8805) -= (490.,20.8805)
	(500.,680.199) += (500.,23.5235) -= (500.,23.5235)
} node [above=0, anchor=east] {Case $T = n^2$ \quad \quad \quad};
\addplot[domain=100:500]{-345.434+45.3126*sqrt(x)} node [below=90, anchor=east] {};% {Fit $-345+45\sqrt{ n }$};
\end{axis}
\end{tikzpicture}
\end{subfigure}
~
\begin{subfigure}[t]{0.3\textwidth}
\centering
\begin{tikzpicture}[scale=0.475]
\begin{axis}[
	xmin = 50, xmax = 550,
	xtick = {100,200,300,400,500},
	ymin = 0, ymax = 300000,
	ytick = {0,100000,200000,300000},
	xlabel=$n$,% ylabel={$\pnorm{ \hat{N} - N }{}$},
	anchor = origin
]

\addplot[mark=x,only marks,error bars/.cd, y dir=both, y explicit] plot coordinates {
	(100.,16295.2) += (100.,1920.78) -= (100.,1920.78)
	(110.,17990.2) += (110.,1472.37) -= (110.,1472.37)
	(120.,20530.9) += (120.,1010.7) -= (120.,1010.7)
	(130.,24521.1) += (130.,1633.29) -= (130.,1633.29)
	(140.,26625.8) += (140.,2014.47) -= (140.,2014.47)
	(150.,33278.4) += (150.,2415.98) -= (150.,2415.98)
	(160.,36977.3) += (160.,1991.87) -= (160.,1991.87)
	(170.,40467.9) += (170.,2199.91) -= (170.,2199.91)
	(180.,45551.5) += (180.,2660.41) -= (180.,2660.41)
	(190.,53018.6) += (190.,4394.48) -= (190.,4394.48)
	(200.,54933.8) += (200.,2808.49) -= (200.,2808.49)
	(210.,63087.9) += (210.,3303.72) -= (210.,3303.72)
	(220.,65440.) += (220.,2901.75) -= (220.,2901.75)
	(230.,75093.9) += (230.,3366.74) -= (230.,3366.74)
	(240.,83452.5) += (240.,4822.04) -= (240.,4822.04)
	(250.,88507.6) += (250.,2210.1) -= (250.,2210.1)
	(260.,96054.4) += (260.,5744.44) -= (260.,5744.44)
	(270.,101447.) += (270.,6424.52) -= (270.,6424.52)
	(280.,110392.) += (280.,3123.74) -= (280.,3123.74)
	(290.,114475.) += (290.,4660.02) -= (290.,4660.02)
	(300.,123855.) += (300.,4794.6) -= (300.,4794.6)
	(310.,132920.) += (310.,5713.48) -= (310.,5713.48)
	(320.,139703.) += (320.,5965.02) -= (320.,5965.02)
	(350.,168665.) += (350.,11945.9) -= (350.,11945.9)
	(375.,193725.) += (375.,5839.36) -= (375.,5839.36)
	(400.,217397.) += (400.,11607.7) -= (400.,11607.7)
	(425.,258607.) += (425.,17371.) -= (425.,17371.)
	(450.,276103.) += (450.,17659.) -= (450.,17659.)	
	(475.,312071.) += (475.,13495.1) -= (475.,13495.1)
	(500.,345445.) += (500.,8760.81) -= (500.,8760.81)	
} node [above=0, anchor=east] {Case $T = n^3$ \quad \quad};
\addplot[domain=100:450]{-81671.4+727.074*x} node [below=90, anchor=east] {};
%\addplot[domain=100:450]{-75596.9 + 695.241*x} node [below=90, anchor=east] {};
\end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Simulations of the asymptotic behavior of $\pnorm{ \hat{N} - N }{}$, together with best fits of the form $c_1 + c_2 \sqrt{ T / n }$ for different scalings of $T$. The simulations suggest that $f(n,T) \approx \sqrt{T/n} = \smallO{T/n}$.}
\label{fig:Asymptotic_behavior_of_spectral_norm_Nhat_minus_N}
\end{figure}

